Bi-directional Contextual Attention for 3D Dense Captioning

3D dense captioning is a task involving the localization of objects and the generation of descriptions for each object in a 3D scene. Recent approaches have attempted to incorporate contextual information by modeling relationships with object pairs or aggregating the nearest neighbor features of an object. However, the contextual information constructed in these scenarios is limited in two aspects: first, objects have multiple positional relationships that exist across the entire global scene, not only near the object itself. Second, it faces with contradicting objectives--where localization and attribute descriptions are generated better with tight localization, while descriptions involving global positional relations are generated better with contextualized features of the global scene. To overcome this challenge, we introduce BiCA, a transformer encoder-decoder pipeline that engages in 3D dense captioning for each object with Bi-directional Contextual Attention. Leveraging parallelly decoded instance queries for objects and context queries for non-object contexts, BiCA generates object-aware contexts, where the contexts relevant to each object is summarized, and context-aware objects, where the objects relevant to the summarized object-aware contexts are aggregated. This extension relieves previous methods from the contradicting objectives, enhancing both localization performance and enabling the aggregation of contextual features throughout the global scene; thus improving caption generation performance simultaneously. Extensive experiments on two of the most widely-used 3D dense captioning datasets demonstrate that our proposed method achieves a significant improvement over prior methods.

==> intro_bak.tex <==
\section{Introduction}
\label{sec:intro}

\bs{
3D dense captioning is a task where we need to 1) localize all objects and 2) generate descriptive sentences for each detected object within a 3D scene.
Early approaches utilized a two-stage process~\cite{chen2021scan2cap, jiao2022more, wang2022spacap3d, zhong2022contextual, cai20223djcg, chen2022d3net, yuan2022xtrans2cap}, where the objects are detected first, then captions are generated afterwards by sequentially feeding the features of each detected object.
Following work~\cite{chen2023vote2capdetr} has borrowed the end-to-end transformer encoder-decoder pipeline from object detection~\cite{carion2020detr} to actively involve contextual information for 3D dense captioning.
In these works, contextual information for predicting relationships are composed by combining object features (e.g., with dot product~\cite{wang2022spacap3d,cai20223djcg} or transformer attention~\cite{chen2023vote2capdetr}) and aggregating local nearest neighbor visual features~\cite{chen2023vote2capdetr}.
% Powered by transformer attentions, this method contextualizes individual objects (i.e., self-attention with other proposals throughout the global scene) to generate dense captions.
% Nevertheless, this pipeline is limited to modeling the relations between object queries, thus fails to fully harness the contextual information that transcends individual object-level representations.

Despite their improved performance, the scope of contextual information in previous 3D dense captioning methods pose its own set of challenges.
First, 3D dense captioning involves positional relationships in respect to the global scene, thus the context scope restricted to the combination of individual objects and their spatially nearest neighbors typically can not provide sufficient information.
 % the intermediate spaces between objects (e.g., union regions~\cite{uniondet} or interaction points~\cite{wang2020learning}) typically could not provide sufficient visual features for capturing relations.
% {\color{red}In 3D scenes, positional relationship within the global scene takes a crucial part, thus requires both intermediate context between the objects and positional relevance to the global scene to correctly identify and describe the object.}
% This is because the relations in 3D dense captioning involves \textit{distractors} (i.e., identical objects with different positional relationship within the scene), which requires global context to correctly identify and describe the object.
% This stands in contrast to 2D scenes, where simple amalgamations of objects (e.g., union regions~\cite{uniondet} or interaction points~\cite{wang2020learning}) suffice to convey contextual relationships.
Next, the endeavor to incorporate contextual features into objects for generating detailed captions encounters a conflicting objective.
This is because the feature representation for the object must encompass precise local features (such as localization or attributes) while simultaneously capturing global context.
Clearly, these challenges limit the performance of 3D dense captioning, which raises an interesting research question-- can we design a transformer architecture that can effectively retrieve the contextual and global features of the 3D scene to facilitate dense captioning without harming object detection?

To this end, we propose {\color{red}MinjungNet}.
{\color{red}MinjungNet} starts from a straightforward extension of previous transformer encoder-decoder architecture~\cite{chen2023vote2capdetr}, where we set a separate set of queries (i.e., Context Query) to versatilely capture the local and global contexts within the 3D scene.
% The context queries are initially voted to non-overlapping areas with existing object proposals.
The disentangled sets of queries resolves the aforementioned contradicting objectives for local and global features, since features that require precise localization boundaries are captured by the original object query while the context query retrieves contextual information spanning the entire scene without adhering to specific localization constraints.
However, we empirically discovered that regions captured with Context Query without any localization objectives lack the integral features for participating instances.
To address this issue, {\color{red}MinjungNet} features a {\color{red}bidirectional feature enhance network (BiFEN)}.
Our proposed {\color{red}BiFEN} first distributes the instance features into the context features according to their attentional relevance.
Then, the contextual features reimbursed with object representations are aggregated back to individual objects according to their newly computed attention scores to generate final dense captions.

Equipped with {\color{red}BiFEN}, {\color{red}MinjungNet} sets a new state-of-the-art standard for 3D dense captioning while simultaneously improving 3D object detection performance.
Extensive experiments on two widely used benchmarks in 3D dense captioning (i.e., ScanRefer~\cite{chen2020scanrefer} and Nr3D~\cite{achlioptas2020referit3d}) show that our proposed {\color{red}MinjungNet} surpasses prior approaches by a large margin.
The contribution of our paper can be summarized as:
\begin{itemize}
    \item We propose a transformer encoder-decoder pipeline that engages 3D dense captioning with two sets of disentangled queries and decoders. This enables our model to simultaneously improve both localization performance while effectively aggregating contextual features to improve relational dense captioning. 
    \item To further improve the quality of contextual features, we propose a novel bidirectional feature enhancer named {\color{red}BiFEN}, where the contextual features are reimbursed with object features and the final dense caption is generated by the combination of the object features and relevant contextual features according to their attention scores.
    \item Our {\color{red}MinjungNet} achieves state-of-the-art performances across multiple evaluation metrics on two most popular benchmark for 3D dense captioning: ScanRefer and Nr3D datasets.
    %two most widely used benchmarks. %3D dense captioning benchmarks.
\end{itemize}

% distractor - , 3D structural information 

% However, incorporating contexts in 3D scenes have its challenges.
% First, unlike 2D images, the intermediate area between objects is usually a void area where the visual features exists in a very sparse manner.
% This differs from 2D scenes where simple unions of objects can represent the `context' of the relation.
% Next, incorporating context features to the objects to generate dense captions presents a contradiction in objectives where the feature representation for the object has to encompass both the accurate local features (e.g., the localization or attributes).

% Dense captioning has to perform precise object localization while generating captions that either independently describe an object's attributes (e.g., a \textit{wooden} chair) or describe the object within its contextual environment (e.g., a chair \textit{in front of} the TV).
% This presents a challenging scenario where the feature representation for a single query must encompass both accurate local features for localization or attribute-based caption generation, alongside incorporating contextual features that dynamically span neighboring regions or the broader global scene.
% Focusing attention on local features can enhance localization and detailed attribute description but reduce sensitivity to the surrounding context. 
% Conversely, spreading attention to include the context can improve understanding of the environmental description but at the cost of localization accuracy.
}

3D dense captioning has been defined in former works~\cite{chen2021scan2cap, chen2022d3net, yuan2022xtrans2cap, wang2022spacap3d, jiao2022more, cai20223djcg, chen2023vote2capdetr} as the task of localizing all the objects in a 3D scene (i.e., object detection) and generating descriptive sentences for each object (i.e., object caption generation).
Early works incorporated a two-stage ``detect-then-describe" pipeline, where we first detect all the object proposals then generate the captions for each object~\cite{chen2021scan2cap, jiao2022more, wang2022spacap3d, zhong2022contextual, cai20223djcg, chen2022d3net, yuan2022xtrans2cap}.
However, the sequential design, lacking sufficient integration of contextual information in these endeavors, has been limited in performance and efficiency.

Succeeding work~\cite{chen2023vote2capdetr} has emulated the transformer encoder-decoder pipeline from object detection~\cite{carion2020detr} to alleviate these issues and fashioned an end-to-end pipeline for 3D dense captioning.
Powered by transformer attentions, this method contextualizes individual objects (i.e., self-attention with other proposals throughout the global scene) to generate dense captions.
Nevertheless, compared to the notable advancements that object detection has experienced, the direct application of this architecture has failed to fully leverage the contextual information required for 3D dense captioning.

Dense captioning has to perform precise object localization while generating captions that either independently describe an object's attributes (e.g., a \textit{wooden} chair) or describe the object within its contextual environment (e.g., a chair \textit{in front of} the TV).
This presents a challenging scenario where the feature representation for a single query must encompass both accurate local features for localization or attribute-based caption generation, alongside incorporating contextual features that dynamically span neighboring regions or the broader global scene.
Focusing attention on local features can enhance localization and detailed attribute description but reduce sensitivity to the surrounding context. 
Conversely, spreading attention to include the context can improve understanding of the environmental description but at the cost of localization accuracy.

In this paper, we propose a pipeline engaging a novel \textit{late aggregation} paradigm called \textbf{SIA (i.e., See It All)}.
Rather than assigning a query \textit{per object} and training them to dynamically incorporate local features, contextual information, and the global scene, SIA allocates a query \textit{per caption}.

\edit{
\begin{itemize}
    \item object feature에 localization과 주변 context까지 모으기를 기대하는 것은 objective가 서로 달라서 어려움.
    \item 이 역할을 둘로 나누기 위해서 instance query와 context query로 나눴음. 그러나 context 특성 상? 또는 benchmark datasets의 구성 상으로 instance feature에는 직접적으로 supervision을 줄 수 있지만 context feature에 직접적으로 주기에는 어려움이 있음.
    \item 각 context feature들은 인접한 instance feature들과 상호작용? 관련?이 있을 것이라고 가정하고, 한 object에 대해서 캡션을 생성할 때 주변 context들과 cross-attention을 해서 attentive context feature를 가져오고, 이 object에 관련있는 attentive context feature와 모든 instance feature들과 cross-attention을 해서 context feature와 관련이 있는 instance feature를 가져오도록 token을 구성함.
    \item xyz 좌표를 기준으로 KNN으로 가져오는 주변 context feature들로 token을 구성했을 때가 성능이 향상하는 것을 통해 이 가설을 증명함.
    \item 또 기존의 voting method에서는 하나의 FFN으로 instance feature와 xyz 좌표 조정을 함께 진행하고, FPS로 좌표를 선별해서 query를 구성함. 우리는 FFN으로 vote feature를 구성하고 거기서 추가로 1 layer를 더해서 좌표 조정을 따로 진행함. (context feature에도 다른 FFN을 적용해서 encoder feature를 재이용하지 않도록 함. 이건 SIA와 다른 점.) query의 역할을 둘로 나누고, center 좌표 생성을 위한 별도의 layer를 추가함으로써 detector의 성능도 향상시킴.
\end{itemize}
}

==> sections/2_Related_work/2_2_vision-language.tex <==
\subsection{Vision-Language}
The research of vision and language has received significant attention in areas such as image captioning \cite{xu2015show,anderson2018bottom,cornia2020meshed,ghandi2022deep}, text-to-image generation \cite{reed2016generative,rombach2022high}, visual grounding \cite{deng2021transvg,fukui2016multimodal}, visual question answering \cite{antol2015vqa}.
Moreover, the introduction of transformers \cite{vaswani2017attention,cornia2020meshed,herdade2019image} marked a transformative phase in this field. Initially developed for language processing, this architecture has achieved significant success in image captioning due to its outstanding ability to understand and generate sequences. Transformer has shown great potential in image captioning when combined with Vision-Language Pretrained (VLP) models. 
Notably, ConZIC \cite{zeng2023conzic} has emerged as an essential model in this field by leveraging the strengths of BERT \cite{devlin2018bert} and CLIP \cite{radford2021learning} to enable controllable zero-shot image captioning, thereby establishing new benchmarks for creation speed and efficiency.

\begin{comment}
Moreover, the introduction of transformers \cite{vaswani2017attention,cornia2020meshed,herdade2019image} marked a transformative phase in the field. Initially developed for a language processing, this architecture achieved considerable success in image captioning due to its outstanding ability to understand and generate sequences. When combined with Vision-Language Pretrained (VLP) models, transformer demonstrated exceptional potential in image captioning. ConZIC \cite{zeng2023conzic} emerged as a crucial model in this area, drawing on the strengths of both BERT \cite{devlin2018bert} and CLIP \cite{radford2021learning} to enable controllable zero-shot image captioning, and thereby establishing a novel benchmark in generation speed and efficiency.
\end{comment}

==> tables/analysis_radius.tex <==
\begin{table*}[t]
   \centering
   \resizebox{\textwidth}{!}{%
     \begin{tabular}{c|cccc}
     \toprule
     \multirow{1}{*}{} & \multicolumn{1}{c}{C@$0.5\uparrow$} & \multicolumn{1}{c}{B-4@$0.5\uparrow$} & \multicolumn{1}{c}{M@$0.5\uparrow$} & \multicolumn{1}{c}{R@$0.5\uparrow$} \\
     \midrule
     \midrule

    \multirow{1}{*}{Instance Query Generator with radius=$0.3$} & \multicolumn{1}{c}{64.75} & \multicolumn{1}{c}{36.76} & \multicolumn{1}{c}{26.23} & \multicolumn{1}{c}{55.63} \\
     
    \multirow{1}{*}{Instance Query Generator with radius=$0.8$} & \multicolumn{1}{c}{56.62} & \multicolumn{1}{c}{34.77} & \multicolumn{1}{c}{24.84} & \multicolumn{1}{c}{52.03} \\   
    
    \midrule
    
    \multirow{1}{*}{Instance Query Generator with radius=$0.3$ \& Anchor Query Generator with radius=$0.8$} & \multicolumn{1}{c}{70.73} & \multicolumn{1}{c}{39.13} & \multicolumn{1}{c}{27.89} & \multicolumn{1}{c}{56.33} \\ 
    
    \multirow{1}{*}{Instance Query Generator with radius=$0.3$ \& Anchor Query Generator with radius=$1.2$} & \multicolumn{1}{c}{\textbf{73.22}} & \multicolumn{1}{c}{\textbf{40.91}} & \multicolumn{1}{c}{\textbf{28.19}} & \multicolumn{1}{c}{\textbf{60.46}} \\
    
     \bottomrule
     \end{tabular}
     }
 \caption{Experimental results of expanding ROI radius in ScanRefer~\cite{chen2020scanrefer} with IoU threshold at $0.5$. C, B-4, M, and R represent the captioning metrics CIDEr \cite{vedantam2015cider}, BLEU-4 \cite{papineni2002bleu}, METEOR \cite{banerjee2005meteor}, and ROUGE-L \cite{chin2004rouge}, respectively.}
 \label{tab:analysis_radius}
 \end{table*} 
